The Event Horizon Telescope Image of the Quasar NRAO 530

We report on the observations of the quasar NRAO 530 with the Event Horizon Telescope (EHT) on 2017 April 5-7, when NRAO 530 was used as a calibrator for the EHT observations of Sagittarius A*. At z=0.902 this is the most distant object imaged by the EHT so far. We reconstruct the first images of the source at 230 GHz, at an unprecedented angular resolution of $\sim$ 20 $\mu$as, both in total intensity and in linear polarization. We do not detect source variability, allowing us to represent the whole data set with static images. The images reveal a bright feature located on the southern end of the jet, which we associate with the core. The feature is linearly polarized, with a fractional polarization of $\sim$5-8% and has a sub-structure consisting of two components. Their observed brightness temperature suggests that the energy density of the jet is dominated by the magnetic field. The jet extends over 60 $\mu$as along a position angle PA$\sim -$28$^\circ$. It includes two features with orthogonal directions of polarization (electric vector position angle, EVPA), parallel and perpendicular to the jet axis, consistent with a helical structure of the magnetic field in the jet. The outermost feature has a particularly high degree of linear polarization, suggestive of a nearly uniform magnetic field. Future EHT observations will probe the variability of the jet structure on ${\mu}$as scales, while simultaneous multi-wavelength monitoring will provide insight into the high energy emission origin.

==> temp.tex <==



























